DeepRepViz: Identifying Confounders in Deep Learning Model Predictions

Deep Learning (DL) models have gained popularity in neuroimaging studies for predicting psychological behaviors, cognitive traits, and brain pathologies. However, these models can be biased by confounders such as age, sex, or imaging artifacts from the acquisition process. To address this, we introduce 'DeepRepViz', a two-part framework designed to identify confounders in DL model predictions. The first component is a visualization tool that can be used to qualitatively examine the final latent representation of the DL model. The second component is a metric called 'Con-score' that quantifies the confounder risk associated with a variable, using the final latent representation of the DL model. We demonstrate the effectiveness of the Con-score using a simple simulated setup by iteratively altering the strength of a simulated confounder and observing the corresponding change in the Con-score. Next, we validate the DeepRepViz framework on a large-scale neuroimaging dataset (n=12000) by performing three MRI-phenotype prediction tasks that include (a) predicting chronic alcohol users, (b) classifying participant sex, and (c) predicting performance speed on a cognitive task called 'trail making'. DeepRepViz identifies sex as a significant confounder in the DL model predicting chronic alcohol users (Con-score=0.35) and age as a confounder in the model predicting cognitive task performance (Con-score=0.3). In conclusion, the DeepRepViz framework provides a systematic approach to test for potential confounders such as age, sex, and imaging artifacts and improves the transparency of DL models for neuroimaging studies.

==> figure_conf.tex <==
\begin{tikzpicture}[scale=1,node distance=1.5cm, 
        trans/.style={thick, <->,shorten >=2pt,shorten <=2pt,>=stealth},]
\node(a) [] {$X$};
\node(b) [right of=a, above of=c] {$c$};
\node(c) [right of=a, below of=b] {$y$};
\draw[red,  ->, densely dashed] (a) -- (b) node[black, midway,left] {$s_c$};
\draw[red, <->, densely dashed] (b) -- (c) node[black, midway,right] {$c \sim y$};
\draw[ ->, thick] (a) -- (c) node[midway,below] {$s_y$};
\end{tikzpicture}
